NECE: Narrative Event Chain Extraction Toolkit

To understand a narrative, it is essential to comprehend the temporal event flows, especially those associated with main characters; however, this can be challenging with lengthy and unstructured narrative texts. To address this, we introduce NECE, an open-access, document-level toolkit that automatically extracts and aligns narrative events in the temporal order of their occurrence. Through extensive evaluations, we show the high quality of the NECE toolkit and demonstrates its downstream application in analyzing narrative bias regarding gender. We also openly discuss the shortcomings of the current approach, and potential of leveraging generative models in future works. Lastly the NECE toolkit includes both a Python library and a user-friendly web interface, which offer equal access to professionals and layman audience alike, to visualize event chain, obtain narrative flows, or study narrative bias.

==> 8-Downstream.tex <==
\section{Question-Answering}
\label{app:dtask_qa}

\textsc{Nece} toolkit is also helpful in enhancing a Question-Answering model's performance on certain narrative events-related questions. 
\citet{xu-etal-2022-fantastic} provided the FairytaleQA dataset, which contains 10,580 QA-pairs annotated by education experts, and conducted benchmark QA experiments with SOTA sequence-to-sequence models. 
The education experts split each story into multiple sections, where each section contains multiple paragraphs. Then, the education experts provided related story section(s) and a category of the question that belongs to an established framework in terms of key narrative elements from educational perspective, along with each QA-pair they annotated. Among the seven categories (character, setting, action, feeling, causal relationship, outcome resolution, and prediction), we notice that action, causal relationship, and outcome resolution are specifically about a certain event or set of events that are causally related. We select those event-related QA-pairs from the original train, valid, and test split, forming three new subsets of 4432/536/513 QA-pairs, respectively. We leverage Rouge-L as the evaluation metric to compare the generated answer with two human-annotated ground-truth answers. 

\begin{table}[!ht]
\centering
\resizebox{.48\textwidth}{!}{%
\small
\begin{tabular}{c||c|c||c|c}
\toprule


 \textbf{Fine-tune}     &   \multicolumn{2}{c||}{ baseline event train split  } &   \multicolumn{2}{c}{\begin{tabular}[l]{@{}c@{}} event valid split  \\ + event sentences\end{tabular} } \\
\midrule
 \textbf{Predict}   &   \begin{tabular}[l]{@{}c@{}} baseline event \\   test split \end{tabular} &   \begin{tabular}[l]{c@{}@{}} event test split  \\ + event sentence\end{tabular} &   \begin{tabular}[l]{@{}c@{}} baseline event \\   test split \end{tabular} &   \begin{tabular}[l]{c@{}@{}} event test split  \\ + event sentence\end{tabular} \\
\midrule
\midrule
\textbf{\begin{tabular}[l]{@{}c@{}} all  \\ event QA\end{tabular}}  &   0.762   &   \textbf{0.765}   &   0.721   &   \textbf{0.732} \\
\midrule
\midrule
\textbf{\begin{tabular}[l]{@{}c@{}} causal  \\ relationship \end{tabular} }   &   0.725   &   \textbf{0.747}   &   0.676   &   \textbf{0.687} \\
\midrule
\textbf{\begin{tabular}[l]{@{}c@{}} outcome  \\ resolution \end{tabular} }   &   0.664   &   \textbf{0.668}   &   0.645   &   \textbf{0.693} \\
\midrule
\textbf{action }               &   0.793   &   \textbf{0.797}   &   0.765   &   \textbf{0.678} \\
 

\bottomrule
\end{tabular}
}

\caption{ The QA experiment result demonstrates our toolkit is able to help models make better predictions on event-related QA-pairs in the FairytaleQA dataset.  }
\vspace{-1em}
\label{tab:qa_experiment}
\end{table}

We hypothesize that providing the more related and informative context for the question would help the model better locate and extract the correct answer.
By leveraging \textsc{Nece}, we can extract events from related story sections of each QA-pair and further identify the sentence(s) containing those events that are closely related to each question based on word vector similarity. Finally, we conduct two experiments to demonstrate the additional information provided by \textsc{Nece} can indeed improve QA model's performance over event-related questions. 

We choose T5~\cite{raffel2020exploring} as the backbone model architecture.
First of all, we fine-tune a baseline T5-base model with the event-related train split and add the event-related sentence that is most relevant to the original input question as additional input during prediction. Compared with the baseline prediction setting, where no additional information is provided, the model's prediction performance improves in all three event-related categories. 

Then, we use \textsc{Nece} and the event-related validation split to fine-tune another model where we concatenate the most closely related sentence and its adjacent sentences as additional information to the original input. During inference, we perform the same prediction experiments described above and observe the model's performance improvement in three event-related categories when we provide the additional input extracted by \textsc{Nece}. Details of the results are shown in Table~\ref{tab:qa_experiment}.

The model backbone for all models fine-tuned for the QA experiment is a T5-base. We maintain the same learning rate of $5e^{-5}$. For the model fine-tuned on event-related train split, we set $epochs=4$. For the model fine-tuned on event-related valid split with additional event information (with about $1/8$ amount of data than the previous setting), we set $epoch=32$. 


==> old/1-Introduction-old.tex <==



\textsc{\sys} extracts structured knowledge about narrative events from an unstructured text corpus. Narrative forms are widely used in both fictional and non-fictional literature to present stories, including fairy-tales, novels, news reports, and memoirs~\citep{carey_snodgrass_2006}. However, the unstructured nature of these texts can make it difficult for readers to quickly comprehend and access the information they need. While many approaches were developed for text processing, including document-level dependency parsing~\citep{mathur-etal-2022-doctime}, document-level semantic parsing~\citep{naseem-etal-2022-docamr}, event-schema induction~\citep{Dror2022ZeroShotOE,Huang2016LiberalEE,li-etal-2020-connecting}, and scripts generation~\citep{Schank1977, Pichotta2015StatisticalSL,chambers-jurafsky-2008-unsupervised, Zhang2021SalienceAwareEC}, there still lacks a tool that combines graphical interface, simplicity, and key narrative features, such as character clustering, gender prediction, and temporal ordering. 

% a format to extract structured knowledge from unstructured narrative corpus


\begin{figure}[tbp]
    \centering
    \includegraphics[width=0.48\textwidth]{images/Salient_event_img.png}
    \caption{The salient events window displays a temporal chain of key events, aiming to offer a succinct event-based representation of the narrative plot}
    \vspace{-0.15in}
    \label{fig:demo_v1}
\end{figure}

This work fills the void by proposing an event chain representation of text, and renders an interface that allows easy access to key temporal and semantic features of any narrative of the user's choice. We choose to use Narrative Event Chain~\citep{chambers-jurafsky-2008-unsupervised,Zhang2021SalienceAwareEC} as the abstract/summarized representation of texts; As defined in \citep{chambers-jurafsky-2008-unsupervised}, narrative event chain has a linear schema made of "partially ordered set of events associated with a protagonist." We expand on the concept to include events associated with all major characters in the narrative, and adopts the salient event concept proposed in ~\citep{Zhang2021SalienceAwareEC} to filter out generic and distracting events. 

% What is narrative Event Chain here? difference from others, especially scripts?

A narrative event chain representation is advantageous for its narrative-central formulation and clearness for visualization. Its linear chain structure not only conveys the temporal order of event occurrence, which is crucial for narrative understanding, but also highlights the actions(events) and actors(characters) that are the backbone of narrative. Compared with parsing graphs, event chain is much more intuitive and readable; and compared with normal script and event-schema, narrative event chain is more optimized for narrative, with events filtering, character clustering, and temporal ordering capabilities. 

% what's the benefit of narrative event chains?

Our toolkit is supported by three main capabilities: 1) extracting and filtering events, 2) extracting narrative features, including main characters, gender of characters, and linking characters to events, and 3) ordering the event chain. We built our pipeline leveraging State of the Art existing tools and novel algorithms. For example, BookNLP~\cite{Bamman2014ABM} package, a toolkit built for document-level narratives, is used for correference-resolution and character clustering. We also apply advanced temporal relation classifiers\citep{Han2021ECONETEC} to order event chains; moreover, we also devised our own gender identification algorithm that supports gender bias detection in event chains. 

% for all characters, including a separate section for gender event chains to facilitate analysis of gender bias in narrative structure.

% We are inspired by the Narrative Event Chain proposed by \citep{chambers-jurafsky-2008-unsupervised}, which defines the chain as "partially ordered set of events associated with the protagonist;" we are also inspired by ~\citep{Zhang2021SalienceAwareEC} for the necessity of filtering out generic/insignificant events. 

%We expand upon previous work by Chambers by including event chains for all characters, not just the protagonist, and simplify the temporal structure to provide a clearer and more accessible temporal interface for users. 




% To provide a more efficient representation that focuses on the core elements of a narrative (characters and events), we propose the use of narrative event chains(a kind of scripts). "A narrative event chain is a partially ordered set of events associated with a character, ordered in the temporal sequence in which they occur"\citep{chambers-jurafsky-2008-unsupervised}. This representation is directly human-readable, and can be used to improve reading comprehension and support various tasks in automatic text processing.


% To address this challenge, researchers have proposed several approaches to improve the representation of narratives, including document-level semantic parsing\citep{naseem-etal-2022-docamr}, event-schema induction\citep{Dror2022ZeroShotOE,Huang2016LiberalEE,li-etal-2020-connecting}, and scripts\citep{Schank1977, Pichotta2015StatisticalSL,chambers-jurafsky-2008-unsupervised, Zhang2021SalienceAwareEC}.



\begin{figure}[tbp]
    \centering
    \includegraphics[width=0.45\textwidth]{images/Character_event.png}
    \caption{The character interface provides event-chains for top-five characters;}
    \vspace{-0.15in}
    \label{fig:demo_character}
\end{figure}

\begin{figure*}[tbp]
    \centering
    \includegraphics[width=1.0 \linewidth]{images/demo_gender_v3.png}
    \caption{The gender page shows event chains for Male, Female, and Mix(plural noun inclusive of all genders). Right hand side showcases a statistics table for most polarized events for both gender meansured by Odds Ratio.}
    \vspace{-3mm}
    \label{fig:demo_gender}
\end{figure*}


We introduce \textsc{Nece}, the first document-level narrative event chain extraction system that boasts an easily accessible online interface. We perform human evaluations to demonstrate the high performance of our character feature extraction, temporal relation classification, and salient event extraction algorithms. Additionally, we demonstrate \textsc{Nece}'s direct application in question-answering systems and its potential for analyzing gender bias in narratives. The \textsc{Nece} toolkit is also motivated by educational purpose to provide aid for narrative understanding, and analysis of potential gender bias in narrative events. Our website is publicly available\footnote{The \textsc{Nece} toolkit is licensed under the MIT license and can be accessed at \url{https://moshi-li.github.io/demo/}}.  A python package is also provided for professionals to harness the various capabilities of \textsc{Nece}, including: 1. Quickly understanding the key plot points of a narrative 2. Detecting gender bias in narrative texts using odds ratios 3. Extracting salient events from a narrative 4. Obtaining document-level temporal orders of events. 


% To provide a simple and accessible interface for learning about narrative events and performing simple bias analysis, we have also created a demo website that is available to the public


% \begin{itemize}
% \item Quickly understanding the key plot points of a narrative
% \item Detecting gender bias in narrative texts using odds ratios
% \item Extracting salient events from a narrative
% \item Obtaining document-level temporal orders of events
% \end{itemize}


==> old/2-System-Design.tex <==


% \begin{figure}[tbp]
%     \centering
%     \includegraphics[width=0.8\textwidth]{images/system.png}
%     \caption{The system design of our pipeline, including the algorithms and packages we run to get the eventual outputs}
%     \vspace{-0.15in}
%     \label{fig:system design pipeline}
% \end{figure}

Researchers and developers can use \textsc{Nece} through a Python package available on GitHub to output the full processing results of a narrative document. The general public can also easily access the toolkit through an online interface to process narrative texts of their choice and interactively find visualizations, analyses, and summaries of the uploaded document. 
% The \textsc{Nece} package allows users to create analysis output files that can be further analyzed. With the online \textsc{Nece} interface, users can visualize character temporal event chains and view associated statistics.

% the right hand section provides statistics of main characters of the narrative.


% \subsection{Related Work}








\subsection{System Pipeline}


%The right-hand section of the gender interface gives a statistical summary of events by gender polarity, as shown in Figure~\ref{fig:bias_gender}



% \begin{figure*}[tbp]
%     \centering
%     \includegraphics[width=1.0 \linewidth]{images/demo_gender_v3.png}
%     \caption{The gender page shows event chains for Male, Female, and Mix(plural nouns that could include both genders).}
%     \vspace{-3mm}
%     \label{fig:demo_gender}
% \end{figure*}




The \textsc{Nece} Toolkit's backend has multiple components running sequentially for each input story. However, each component module can be run individually if the necessary intermediate files already exist. The main component modules are summarized in Figure\ref{fig:sys_pipeline} where the orange coloring represents an existing toolkit and the blue coloring represents our new contributions. Some key components are explained in more detail below. 
 
\#1. Character Extraction: A modified version of BookNLP \cite{Bamman2014ABM} extracts and clusters characters and performs co-reference resolution to link pronouns to characters. We use the BookNLP output to count the combined name mentions and pronoun mentions for characters to arrive at their relative importance category, and a high-level categorization as primary, secondary, and tertiary characters.

\#2. Event Extraction and Semantic Role Labeling: We identify events with AllenNLP's \cite{Gardner2017AllenNLP} Semantic Role Labeling (SRL) model which extracts verb events and their related arguments such as subject and direct object. Additionally, we determine salient events, those most important to main plot, using our novel algorithm based on the tf-idf (term frequency–inverse document frequency) algorithm. 

\#5. Temporal Event Ordering: The extracted verb events are filtered and read into ECONET \cite{Han2021ECONETEC} to find the temporal relationship between pairs of events. A custom ranking algorithm then orders all events based on their pairwise relationships.

\begin{figure*}[tbp]
  \centering
  \includegraphics[width=1.0\linewidth]{images/new_pipeline.png}
  \caption{The system design pipeline for \textsc{Nece} Toolkit; orange coloring denotes models and code from existing packages; blue coloring represents our novel algorithms.}
  \label{fig:sys_pipeline}
\vspace{-3mm}
\end{figure*}



\#6. Character Gender Extraction: The character and co-reference resolution output from Step \#1 is used in combination with NLTK's parts of speech tagging to extract gender features of characters. Due to limitations of current method, we only offer an imperfect gender categorization as female, male, group/non-binary, or unknown (See Limitation~\ref{sec:limits}) 
%Characters are categorized as primary, secondary, and tertiary characters as determined by their number of appearances.

\#7. Salient events are defined as events that are relevant, or essential, to the main narrative of the story as defined by ~\citep{Zhang2021SalienceAwareEC}. To find the salient events, we trained an inverse document frequency(idf) dictionary on a fairy-tale corpus~\citep{xu-etal-2022-fantastic} to calculate a tf-idf based salience score. Inverse document frequency can filter out generic events, and document frequency can be used to identify locally important events in the analyzed text. Our experiments ~\ref{event_chain_table} show that a weighted tf-idf score for the stem words of events successfully identifies salient events. 
\begin{figure}[tbp]
    \centering
    \includegraphics[width=0.45\textwidth]{images/demo_character_v3.png}
    \caption{The character interface provides event-chains for top-five characters;}
    \vspace{-0.15in}
    \label{fig:demo_character}
\end{figure}

\textbf{Other Key Event Extraction Methods} RAKE \citep{rakeinbook} is a common method to extract keywords from documents by creating an undirected and unweighted graph of candidate keywords, and only output the ones have the top co-occurrence. Another well-know unsupervised keyword extraction method is YAKE \citep{CAMPOS2020257}. YAKE uses local statistical features to identify informative content within the text, with with which it calculates an importance of single terms, along with a relevance score determined by an N-gram model,YAKE outputs a list of top keywords. 


\#8.  Temporal Event Chains of Characters: While temporal relations between events are much more complicated than a linear event chain, we still choose an imperfect global event chain representation due to its simplicity in aggregating and summarizing hundreds of events. We acknowledge, as pointed out by ~\citep{NingWuRo18}, not all events are aligned on the same temporal axis and thus are not comparable. However, we show through human evaluation that our simplified event chain is a more accurate temporal model than using sequential ordering based merely on the event's position in the narrative. 

\#9. Statistic Calculations: These aggregate statistics offer an overview of the narrative document at the character-level, event-level, and story-level. The statistics include metrics for quantifying bias between characters of different narrative importance or between male and female characters. It displays the importance category as reported in \# 1; The bias metric is the odds ratio as the as calculated using ~\citep{Sun2021MenAE, monroe_colaresi_quinn_2017}. For example, in a given story, the occurrence of the event 'kill' has an odds ratio of four from male to female characters. This means that male characters are four times more likely than female characters to be involved in an event involving killing. We apply a common correction, Haldane-Anscombe~\citep{Lawson2004OddsRatio}, to account for cases in which one group has no observed counts of the event. 




% Character-level, event-level, and story-level aggregate statistics are calculated which include odds ratios between female and male characters. 


% \subsection{Python Package}
% \label{subsec:sys_package}

% The Toolkit Python package runs the pipeline and creates analysis files from a story input. The main table analysis files are a character attributes table and ranked temporal events by character table. Output files are created with character-level, event-level, and story-level statistics.  These files can be leveraged by the user to conduct their own analyses on the individual story or on a corpus of stories. 

%The character attributes table contains a row for each character and their character attributes such as co-reference ID, names, number of appearances, gender, extracted gender certainty score, and character importance (primary, secondary, or tertiary). The character temporal events table contains a row for each event in which a character is involved as a subject or direct object. The row includes the event verb, the character co-reference ID, the character argument (subject or direct object), sentence ID, event and argument locations in the text, and character attributes. Output files are created with character-level, event-level, and story-level statistics. These include contingency tables of event counts by character gender and importance and by argument (subject and direct object), the top events for female and male characters, and odds ratios between events by character gender and importance. These files can be leveraged by the user to conduct their own analyses on the individual story or on a corpus of stories. These include contingency tables of event counts by character gender and importance and by argument (subject and direct object), the top events for female and male characters, and odds ratios between events by character gender and importance.
\input{table_2}

\subsection{Online Interface}
\label{subsec:sys_ui}
The online toolkit interface takes in story text as input and creates a visualization of the event chains and maps the events back to the text in a dynamic graphical interface. As shown in Figure\ref{fig:demo_v1}, annotated story text occupies the main screen and users can scrolled up and down for full content; on the lower left part of the screen is the event chain where clicking on the event block directs the user to the annotated event in the text corpus. For the Gender and Character feature windows, a statistics overview is offered on the right hand section of the screen. 

% Character event chains are visualized as interactive graphs on the left of the interface. Statistics are displayed as interactive tables and plots on the right. Users can choose to view the character event chains by salient events, gender, and individual character. 

\subsubsection{Salient Event Chain}
% \textbf{This part's UI will be lead by Moshi}

The first feature of our interface, salient event chain extraction and visualization, is depicted in Figure \ref{fig:demo_v1}. While a complete event chain can be helpful to a get holistic and comprehensive view of the story, long event chains can be hard to digest for users. Thus, we focus on the salient events of which main characters are participants. The event chain is organized in the temporal order by which the event happens. When clicking on one of the events, the user is taken to the location of the event in the text with the subject and objects of the event highlighted.

% While a complete event chain can be helpful to get holistic and comprehensive view of the story, long event chains can be hard to digest for users. Moreover, too many events will make creation of event chain harder, by having so many events in a sentence. So, we designed an algorithm based on TF-IDF to extract salient events in which each sentence can have at most one salient event. An event chain will be created to display this salient events chain, if the user click on the Salient button. 


\subsubsection{Gender}
\label{subsec:interface_attr}
% \textbf{This part is led by Toye}


% \begin{figure*}[tbp]
%   \centering
%   \includegraphics[width=1.0\linewidth]{images/new_pipeline.png}
%   \caption{The system design pipeline for \textsc{Nece} Toolkit; orange coloring denotes models and code from existing packages; blue coloring represents our novel algorithms.}
%   \label{fig:sys_pipeline}
% \vspace{-3mm}
% \end{figure*}



% So, we also created separate event chains that are tailor to a gender group or one main character, by clicking on the gender and character button. The create event chain will be shorter, and only relevant to the selected character or gender group. Specific design for gender and character interfaces are described in the following.

% When the user enters the gender interface, they can select either male, female, or non-gendered, where non-gendered refers to characters that contain both males and females. The gender interface will generate story level statistics about events related to that selected gender, including top gender characters, number of appearances of those characters, what are the features of events related to that character. Lastly, a event-chain related to this gender group will be produced, and users can click into events to find its location in the story text. 
%, where score greater than 1.96 is considered statistically significant
% To call attention to fairness in print media, book review website KIRKUS enacted policy to requires all reviews to explicitly mention the race of characters. 

Gender representation in print media has attained increasing public attention: according to ~\citep{mccabe2011childrensbooks}, no more than 33\% of children's books published in any given year contain female main characters, the number is up to 100\% for male characters. Following the call to emphasize gender fairness by explicitly identifying the gender of main characters of books\footnote{https://www.kirkusreviews.com/news-and-features/articles/unmaking-white-default/}, we present event chains for different gender groups, as shown in Figure~\ref{fig:demo_gender}. We use different shapes to denote the argument type of the character(subject or direct object) of the event; different coloring denotes the gender of the subject argument of events. The statistics section displays a contingency table of the story-level event statistics for the most gender polarized events based on odds ratio. 
% by character attribute and argument. It also displays the top events for female and male characters as determined by our bias metric, odds-ratio. Selecting a node in the event graph pulls up additional information for that particular event, including location in the story text, other occurrences in the event chain, gender bias, and character importance bias.

% Each event's shape denotes the argument of the event (subject or direct object) while different coloring designates the gender of the character in the argument of the event. 



\subsubsection{Character}
\label{subsec:interface_char}
% \textbf{This part is led by Toye}
% Character interface will create a table of the top characters in the story, and their gender, importance, and related events. If the user clicks into a character, they will be able to see an event-chain created for that character. On the right side of the screen, there will also be story-level meta-statistics about the character in the story. 
The character feature, shown in Figure~\ref{fig:demo_character}, displays option tabs for the top 5 characters in the narrative as determined by number of appearances. Clicking on the tab brings the respective event chains and a statistics table summarizing the importance of characters by mentions in the story. 


% This tab pulls up a table displaying every character and their attributes. Clicking on an individual character displays that character's event chain. As in the Gender screens, clicking on an event in the chain shows additional information and statistics about the event. 

% \begin{figure}[tbp]
%     \centering
%     \includegraphics[width=0.5\textwidth]{images/character.png}
%     \caption{The system design of our pipeline, including the algorithms and packages we run to get the eventual outputs}
%     \vspace{-0.15in}
%     \label{fig:character_interface}
% \end{figure}



